Test-time Adaptation in the Dynamic World with Compound Domain Knowledge Management

Prior to the deployment of robotic systems, pre-training the deep-recognition models on all potential visual cases is infeasible in practice. Hence, test-time adaptation (TTA) allows the model to adapt itself to novel environments and improve its performance during test time (i.e., lifelong adaptation). Several works for TTA have shown promising adaptation performances in continuously changing environments. However, our investigation reveals that existing methods are vulnerable to dynamic distributional changes and often lead to overfitting of TTA models. To address this problem, this paper first presents a robust TTA framework with compound domain knowledge management. Our framework helps the TTA model to harvest the knowledge of multiple representative domains (i.e., compound domain) and conduct the TTA based on the compound domain knowledge. In addition, to prevent overfitting of the TTA model, we devise novel regularization which modulates the adaptation rates using domain-similarity between the source and the current target domain. With the synergy of the proposed framework and regularization, we achieve consistent performance improvements in diverse TTA scenarios, especially on dynamic domain shifts. We demonstrate the generality of proposals via extensive experiments including image classification on ImageNet-C and semantic segmentation on GTA5, C-driving, and corrupted Cityscapes datasets.

==> table/settings.tex <==
{\renewcommand{\arraystretch}{1.1}
\begin{table*}[t]\centering
\caption{\textbf{Comparison of settings to mitigate the domain shift.} Domain labels indicate whether the domain information exists for target samples. Offline indicates that all target data are available prior to model deployment. In contrast, online refers to encountering target samples in a streaming fashion. Know. manage. denotes knowledge management of sub-target domains. }
\vspace{-.5em}
\resizebox{0.99\textwidth}{!}{ 
\begin{tabular}{l c c c c c c}
\toprule
Setting                & Source / Target  & Target domain & Target State  & Domain label & Know. manage.\\ 
\drule
Unsupervised domain adaptation~\cite{ganin2015unsupervised}  & labeled  / unlabeled                                   & single    & offline           & Yes                          & No                                                 \\
Compound domain adaptation~\cite{liu2020open}      & labeled  / unlabeled                                   & multiple  & offline            & Yes                 & No                                                        \\
Test-time adaptation~\cite{tent}      & unknown / unlabeled                          & single    & online          & Yes                            & No                                       \\
Continual test-time adaptation~\cite{ecotta}             & unknown / unlabeled       & multiple  & online              & No                & No                                  \\
\gr
Cyclical compound domain test-time adaptation & unknown / unlabeled  & multiple  & online                            & No  & Yes                         \\
\toprule
\end{tabular}}
\label{table:settings}
\vspace{-1.8em}
\end{table*}}


==> table/test_teble.tex <==
\begin{table}
\begin{center}
\vspace{-.1em}
\tablestyle{3pt}{1.1}
\scriptsize{
\begin{tabular}{l y{32}z{18}x{14}x{14}x{14}x{16}x{16}x{16}x{16}}
Backbone & Method & FLOPS & AP$^\textsuperscript{box}$ & AP$^{\textsuperscript{box}}_{50}$ & AP$^{\textsuperscript{box}}_{75}$ & AP$^\textsuperscript{mask}$ & AP$^{\textsuperscript{mask}}_{50}$ & AP$^{\textsuperscript{mask}}_{75}$ \\
\shline
\scriptsize ConvNeXt V1-B & Supervised & 486G & 50.3 & 71.6 & 56.1 & 44.9 & 68.5 & 48.8 \\
\baseline{ConvNeXt} V2-B & Supervised & 486G & 51.0 & 72.4 & 56.6 & 45.6 & 69.5 & 49.7 \\
\gc{Swin-B} & SimMIM & 497G & 52.3 & $-$ & $-$ & $-$ & $-$ & $-$  \\
\gr
ConvNeXt V2-B & dd & 486G & \textbf{52.9} & 72.6 & 58.9 & \textbf{46.6} & 70.0 & 51.1 \\
\hline
ConvNeXt V1-L & Supervised & 875G & 50.6 & 71.5 & 56.3 & 45.1 & 68.7 & 49.2 \\
ConvNeXt V2-L & Supervised & 875G & 51.5 & 72.5 & 57.3 & 45.8 & 69.4 & 49.9 \\
Swin-L & SimMIM & 904G & 53.8 & $-$ & $-$ & $-$ & $-$ & $-$ \\
\gr
ConvNeXt V2-L & dd & 875G & \textbf{54.4} & 73.9 & 60.4 & \textbf{47.7} & 71.4 & 52.3 \\
\hline
Swin V2-H & SimMIM & $-$ & 54.4 & $-$ & $-$ & $-$ & $-$ & $-$ \\
\gr
ConvNeXt V2-H & dd & 2525G & \textbf{55.7} & 75.2 & 61.8 & \textbf{48.9} & 72.8 & 53.6
\end{tabular}
\vspace{-.5em} }
\end{center}
\caption{\textbf{COCO object detection and instance segmentation results} using Mask-RCNN. FLOPS are calculated with image size (1280, 800). Swins’ results are from. All COCO fine-tuning experiments rely on ImageNet-1K pre-trained models.}
\label{tab:coco_transfer}
\end{table}
